On the SDEs and Scaling Rules for Adaptive Gradient Algorithms

Approximating Stochastic Gradient Descent (SGD) as a Stochastic Differential Equation (SDE) has allowed researchers to enjoy the benefits of studying a continuous optimization trajectory while carefully preserving the stochasticity of SGD. Analogous study of adaptive gradient methods, such as RMSprop and Adam, has been challenging because there were no rigorously proven SDE approximations for these methods. This paper derives the SDE approximations for RMSprop and Adam, giving theoretical guarantees of their correctness as well as experimental validation of their applicability to common large-scaling vision and language settings. A key practical result is the derivation of a $\textit{square root scaling rule}$ to adjust the optimization hyperparameters of RMSprop and Adam when changing batch size, and its empirical validation in deep learning settings.

==> experiments.tex <==
\kaifeng{Question: should we split this section into two subsections, and move them into Section 5 and 6 respectively?}

%We corroborate the relevance of \Cref{thm:rmsprop_sde,thm:adam_sde} to common deep learning settings by running the Adam SVAG algorithm (\Cref{def:svag_alg}) on CIFAR-10 \cite{cifar10} with ResNet-50 \cite{he2015delving} for up to $\ell=8$ and comparing the simulated SDE trajectory to the discrete one (i.e., $\ell=1$). Recall that the notion of approximation between stochastic processes (see \Cref{def:weak_approx}) relies on several test functions being close. We use the mathematically well-behaved test functions $\Tr(\mSigma(\vtheta_k))$ and $\|\vg_k\|$ as well as the more practically relevant train and test accuracies (which are not differentiable, and thus not covered by the theory). In \Cref{fig:adamsvag,fig:rmspropsvag}, we observe that the converged SVAG trajectories are close to the original discrete ones according to these test functions. These findings suggest that standard deep learning settings may have a well-behaved NGOS (\Cref{def:NGOS,as:f}) that satisfies the bounded moment conditions (\Cref{def:bound-moment}), thereby allowing \Cref{thm:svag} to apply. 
%In particular, heavy-tailed noise is not crucial in these settings.

We also test the square root scaling rule directly on RoBERTa-large
\cite{liu2019roberta} trained on the Wiki+Books corpus \cite{zhu2015aligning}
and ResNet-50 trained on ImageNet \cite{deng2009imagenet}. See
\Cref{fig:largescaleexpts_mainpaper}. To make language model
training efficient, we use the Academic BERT recipe outlined in
\cite{izsak2021how}. 
%We consider the scaling rule a success when the test accuracies are within a 3\% range at different hyperparameter settings along the scaling rule. 
%\abhishek{Some details about the settings on ImageNet and language models}
%We compare the square root scaling rule to a linear scaling on the same settings and find that the square root scaling can match the well-behaved mathematical test functions and the more practically used test accuracy better than the linear scaling can.




  
 \iffalse 
\begin{table}
\centering
\begin{tabular}{c|c|c|c}
		$B$ & Square Root  & Linear &  None \\ \hline
		$8192$ &  $91.06$ & $90.65$ & $87.13$\\
		$16384$ &  $90.74$ & $88.9$ & $87.48$\\
		%\hline\hline 
		%RoBERTa-Large on Wiki+Books & X & X & X
\end{tabular}
\caption{
Applying linear scaling rule or no scaling rule to ResNet-50 trained on CIFAR-10 using Adam results in worse generalization performance, especially at very large batch sizes. The baseline performance is $92.37$ with batch size $256$. We apply the square root, linear, and no scaling rules to set the hyperparameters when training with batch sizes $8192$ and $16384$.}
\label{tab:sqrt_vs_linear_cifar}
\end{table}
\fi 

%\abhishek{Write some more details here.}

 \iffalse 
\begin{figure*}[!htbp]
%\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\linewidth]{Expts_files/adamsvag.png}}
\caption{Adam SVAG with Resnet50 on CIFAR-10}
\label{fig:adamsvag}
\end{center}
%\vskip -0.2in
\end{figure*}


\begin{figure*}[!htbp]
%\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\linewidth]{Expts_files/rmspropsvag.png}}
\caption{RMSprop SVAG with Resnet50 on CIFAR-10}
\label{fig:rmspropsvag}
\end{center}
%\vskip -0.2in
\end{figure*}
\fi 













